Semantically Driven Auto-completion

The Bloomberg Terminal has been a leading source of financial data and analytics for over 30 years. Through its thousands of functions, the Terminal allows its users to query and run analytics over a large array of data sources, including structured, semi-structured, and unstructured data; as well as plot charts, set up event-driven alerts and triggers, create interactive maps, exchange information via instant and email-style messages, and so on. To improve user experience, we have been building question answering systems that can understand a wide range of natural language constructions for various domains that are of fundamental interest to our users. Such natural language interfaces, while exceedingly helpful to users, introduce a number of usability challenges of their own. We tackle some of these challenges through auto-completion for query formulation. A distinguishing mark of our auto-complete systems is that they are based on and guided by corresponding semantic parsing systems. We describe the auto-complete problem as it arises in this setting, the novel algorithms that we use to solve it, and report on the quality of the results and the efficiency of our approach.

==> sections/experiments-app.tex <==
% !TEX root = ../main.tex

\section{Additional Experiments} \label{app-experiments}
\subsection{Predictiveness}
We extend the Predictiveness experiments presented in Section \ref{predictiveness-exp} with a more fine-grained analysis
of predictiveness based on query prefix lengths. Figure \ref{predictiveness-per-length} shows the results for the weighted
and unweighted MRR and MPMRR measures for prefixes of lengths between 3 and 20 characters. Using the MPMRR measure, we
can see that predictiveness is high for all prefix lengths. However, the domains exhibit different behavior in terms of the
relation between length and predictiveness and the gap between MPMRR and MRR, which we discuss below.

\begin{figure}[h]
   \centering
   \includegraphics[width=0.35\textwidth]{figures/mrrperlength}\\

   \caption{Predictiveness as function of prefix length.}
  \label{predictiveness-per-length}
\end{figure}

In BNDS predictiveness improves with length. This is because as the query becomes 
more specific, and provides more ranking context, the system is better able to zoom in on the desired completion. In news, things are
somewhat different. There is steady improvement until around 10 characters, and then the numbers fall. EXPLANATION.


\subsection{Efficiency}

Figure \ref{efficiency-per-length} shows a plot of average completion time for various 
prefix lengths for each of our domains. The times observed for BNDS increase slightly 
with prefix length. In NEWS there is a pronounced drop in time as the prefixes 
become longer.  EXPLANATION

\begin{figure}[h!]
   \centering
   \includegraphics[width=0.35\textwidth]{figures/timeperlength}\\

   \caption{Completion time as function of prefix length.}
  \label{efficiency-per-length}
\end{figure}




